Uncertainty-driven Exploration Strategies for Online Grasp Learning

Existing grasp prediction approaches are mostly based on offline learning, while, ignoring the exploratory grasp learning during online adaptation to new picking scenarios, i.e., objects that are unseen or out-of-domain (OOD), camera and bin settings, etc. In this paper, we present an uncertainty-based approach for online learning of grasp predictions for robotic bin picking. Specifically, the online learning algorithm with an effective exploration strategy can significantly improve its adaptation performance to unseen environment settings. To this end, we first propose to formulate online grasp learning as an RL problem that will allow us to adapt both grasp reward prediction and grasp poses. We propose various uncertainty estimation schemes based on Bayesian uncertainty quantification and distributional ensembles. We carry out evaluations on real-world bin picking scenes of varying difficulty. The objects in the bin have various challenging physical and perceptual characteristics that can be characterized by semi- or total transparency, and irregular or curved surfaces. The results of our experiments demonstrate a notable improvement of grasp performance in comparison to conventional online learning methods which incorporate only naive exploration strategies. Video: https://youtu.be/fPKOrjC2QrU

==> name.tex <==
import os, sys
import pandas as pd
import seaborn as sns
from matplotlib import pyplot
import matplotlib.pyplot as plt
import numpy as np
import argparse
from datetime import datetime
import time, glob, csv
import pandas as pd

# time
current_time = time.time()
# set sns style
sns.set(style="darkgrid", font_scale=1.5)


# helpers
def smooth(scalars, weight):  # Weight between 0 and 1
    last = scalars[0]  # First value in the plot (first timestep)
    smoothed = list()
    for point in scalars:
        smoothed_val = last * weight + (1 - weight) * point  # Calculate smoothed value
        smoothed.append(smoothed_val)                        # Save it
        last = smoothed_val                                  # Anchor the last smoothed value

    return smoothed

def create_lineplot(df, a4_dims, current_time, tag = None, abl=False):
    temp_ = df
    print (temp_.head())
    fig, ax = pyplot.subplots(figsize=a4_dims)
    sns.lineplot(data=temp_, x="Step", y="Success Rate", hue="Method" if not abl else "Online training steps") # turn this into error_bar="se", standardeviation of the mean estimator
    
    plt.legend(loc='best').set_draggable(True)
    

    xscale = np.max(np.asarray(temp_['Step'])) > 5e3
    if xscale:
        # Just some formatting niceness: x-axis scale in scientific notation if max x is large
        plt.ticklabel_format(style='sci', axis='x', scilimits=(0,0))
    plt.tight_layout(pad=0.5)
    str_time = datetime.utcfromtimestamp(current_time).strftime('%Y-%m-%d_%H:%M:%S')
    fig.savefig(f"{tag}.png")
    
def create_barplot(df, a4_dims, current_time, tag = None, bottom = 0.35, abl = False):
    temp_ = df
    print (temp_.head())
    fig, ax = pyplot.subplots(figsize=a4_dims)
    splot = sns.barplot(data=temp_, x="Method" if not abl else "Online training steps", 
                        y="Success Rate", width=.5
                        #, errorbar=("pi", 30)
                        , capsize=.2
                        , ci=None if abl else "deprecated"
                        ) # turn this into error_bar="se", standardeviation of the mean estimator
    axes = splot.axes
    axes.set_ylim(bottom, 1.0)
   
    for g in splot.patches:
        splot.annotate(format(g.get_height()*100, '.1f')+"%",
                    (g.get_x() + g.get_width() / 2., (g.get_height() + bottom) / 2.),
                    ha = 'center', va = 'bottom',
                    xytext = (0, 9),
                    textcoords = 'offset points')
        
    plt.legend(loc='best').set_draggable(True)

    xscale = np.max(np.asarray(temp_['Step'])) > 5e3
    if xscale:
        # Just some formatting niceness: x-axis scale in scientific notation if max x is large
        plt.ticklabel_format(style='sci', axis='x', scilimits=(0,0))
    plt.tight_layout(pad=0.5)
    str_time = datetime.utcfromtimestamp(current_time).strftime('%Y-%m-%d_%H:%M:%S')
    if abl:
        sns.lineplot(data = temp_, marker='o',x="Method" if not abl else "Online training steps", y="Success Rate")
    fig.savefig(f"{tag}.png")

def parse_args():
    parser = argparse.ArgumentParser()
    parser.add_argument('--width', default=11.7, type=float)
    parser.add_argument('--height', default=10, type=float)
    args = parser.parse_args()
    return args

def main(qua, abl = False, group=False):

    args = parse_args()
    a4_dims = (args.width, args.height)


    step_list = []
    success_rate_list = []
    episode_list = []
    method_list = []

    path = "experiments.xls"
    df = pd.ExcelFile(path)
    METHOD_LIST = df.sheet_names
    Quantile_LIST =[a for a in METHOD_LIST if "quan" in a]
    MV_LIST =[a for a in METHOD_LIST if not "quan" in a]
    METHOD_LIST = Quantile_LIST if qua else MV_LIST
    if group:
        abl = False
        METHOD_LIST = ["offline", "online", "online ucb epi ada", "online ucb epi"]
        tags = "epi_"
        if qua:
            METHOD_LIST = [a+" quantile" for a in METHOD_LIST]
            tags = "epi_quantile_"
    else:
        if not qua:
            tags = "epi_ada_" if abl else "MV_" 
        else:
            
            tags = "epi_quantile_ada_" if abl else "QR_"

    for using_method in METHOD_LIST:
        if using_method =='total':
            continue
        elif not group and 'ada' in using_method:
            continue
        
        try:
            int(using_method[0])
            if not abl:
                continue
        except:
            if abl:
                continue
        
                
        
        success_rate_method_list = pd.read_excel(path, using_method, header=None).T.astype('float32').values.tolist()
        
        # using_method += " steps" if abl else ""
        for episode_index, success_rate_episode in enumerate(success_rate_method_list):
            for step_index, success_rate in enumerate(success_rate_episode):
                step_list.append(step_index + 1)
                success_rate_list.append(success_rate)
                episode_list.append(episode_index)
                method_list.append(using_method[:-8] if qua else using_method)

    temp_df = pd.DataFrame(list(zip(step_list, success_rate_list, episode_list, method_list)), \
                                    columns=['Step', 'Success Rate', "Episode", "Method" if not abl else "Online training steps"])
    final = temp_df[temp_df['Step'] == 24]

    print (temp_df.head())
    
    temp_df = temp_df.sort_values(by ='Method' if not abl else "Online training steps").sort_index()
    final = final.sort_values(by ='Method' if not abl else "Online training steps").sort_index()
    create_lineplot(temp_df, a4_dims, current_time, f"{tags}line" , abl=abl)
    create_barplot(final, a4_dims, current_time, f"{tags}bar",abl=abl)
    plt.clf()

if __name__ == '__main__':
    main(abl=True, qua=False)
    main(abl=True, qua=True)
    main(abl=False, qua=True)
    main(abl=False, qua=False)
    main(group=True, qua=False)
    main(group=True, qua=True)


    

